Quasi-Equivalence Discovery for Zero-Shot Emergent Communication

Effective communication is an important skill for enabling information exchange in multi-agent settings and emergent communication is now a vibrant field of research, with common settings involving discrete cheap-talk channels. Since, by definition, these settings involve arbitrary encoding of information, typically they do not allow for the learned protocols to generalize beyond training partners. In contrast, in this work, we present a novel problem setting and the Quasi-Equivalence Discovery (QED) algorithm that allows for zero-shot coordination (ZSC), i.e., discovering protocols that can generalize to independently trained agents. Real world problem settings often contain costly communication channels, e.g., robots have to physically move their limbs, and a non-uniform distribution over intents. We show that these two factors lead to unique optimal ZSC policies in referential games, where agents use the energy cost of the messages to communicate intent. Other-Play was recently introduced for learning optimal ZSC policies, but requires prior access to the symmetries of the problem. Instead, QED can iteratively discovers the symmetries in this setting and converges to the optimal ZSC policy.

==> acknowledgements.tex <==
\iffalse
If a paper is accepted, the final camera-ready version will (and probably should) include acknowledgments. Add here thanks to reviewers who gave useful comments and to colleagues who contributed.
Different conferences have different instructions regarding funding agencies and corporate sponsors that provided financial support (sometimes in the first page, sometimes in the acknowledgments).
\fi


%We would like to thank Franziska Meier for useful discussions and feedback on paper drafts. 
